SwishNet: A Fast Convolutional Neural Network for Speech, Music and Noise Classification and Segmentation

Speech, Music and Noise classification/segmentation is an important preprocessing step for audio processing/indexing. To this end, we propose a novel 1D Convolutional Neural Network (CNN) - SwishNet. It is a fast and lightweight architecture that operates on MFCC features which is suitable to be added to the front-end of an audio processing pipeline. We showed that the performance of our network can be improved by distilling knowledge from a 2D CNN, pretrained on ImageNet. We investigated the performance of our network on the MUSAN corpus - an openly available comprehensive collection of noise, music and speech samples, suitable for deep learning. The proposed network achieved high overall accuracy in clip (length of 0.5-2s) classification (>97% accuracy) and frame-wise segmentation (>93% accuracy) tasks with even higher accuracy (>99%) in speech/non-speech discrimination task. To verify the robustness of our model, we trained it on MUSAN and evaluated it on a different corpus - GTZAN and found good accuracy with very little fine-tuning. We also demonstrated that our model is fast on both CPU and GPU, consumes a low amount of memory and is suitable for implementation in embedded systems.

==> tab_segrecall.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet5'
\begin{table}[tbp]
	\centering
	\caption{Frame-wise Recall For a Contextual Window Length of 0.5s}
	\begin{tabular}{p{7.5em}P{3em}P{3em}P{3em}P{3em}}
		\toprule
		\textbf{Network} & \textbf{Noise Recall} & \textbf{Music Recall} & \textbf{Speech Recall} & \textbf{Average Recall} \\
		\midrule[1pt]
		\textbf{GMM} & 73.05\% & 98.57\% & 99.67\% & 90.43\% \\
		\midrule
		\textbf{SNN} & 73.05\% & 98.57\% & 99.67\% & 90.43\% \\
		\midrule
		\textbf{SwishNet-slim} & 73.05\% & 98.57\% & 99.67\% & 90.43\% \\
		\midrule
		\textbf{SwishNet-wide} & 78.08\% & 98.84\% & 99.69\% & 92.20\% \\
		\midrule
		\textbf{MobileNet} & 87.76\% & 99.63\% & 99.63\% & 95.67\% \\
		\bottomrule
	\end{tabular}%
	\label{tab:segrecall}%
\end{table}%
